CANTO -- Covert AutheNtication with Timing channels over Optimized traffic flows for CAN

Previous research works have endorsed the use of delays and clock skews for detecting intrusions or fingerprinting ECUs on the CAN bus. Similar techniques have been also proposed for establishing a time-covert cryptographic authentication channel, in this way cleverly removing the need for cryptographic material inside the limited payload of CAN frames. The main shortcoming of such works is the limited security level that can be achieved under normal CAN-bus traffic. In this work we endeavour to test the limits of the achievable security level by relying on optimization algorithms for scheduling CAN frames. Under practical bus allocations that are based on real-world scenarios, we are able to extract around 4--5 bits of authentication data from each frame which leads to an efficient intrusion detection and authentication mechanism. By accumulating covert channel data over several consecutive frames, we can achieve higher security levels that are in line with current security demands. To prove the correctness of our approach, we present experiments on state-of-the-art automotive-grade controllers (Infineon Aurix) and bus measurements with the use of industry standard tools, i.e., CANoe.

==> analysis.tex <==
\section{Analysis of clock accuracy in automotive-grade controllers}

\def\spicw{2.8}
\def\lpicw{4.5}
\def\clpicw{6}

\newcommand\clock{\mathcal{C}}
\newcommand\offset{\mathcal{O}}
\newcommand\refr{\star}
\newcommand\real{\mathrm{ideal}}
\newcommand\med{\mathrm{med}}
\newcommand\mean{\mathrm{mean}}
\newcommand\mmin{\mathrm{min}}
\newcommand\fmed{\mathsf{Median}}
\newcommand\fmean{\mathsf{Mean}}
\newcommand\fmin{\mathsf{Min}}
\newcommand\vmed{v_\mathsf{med}}
\newcommand\vmean{v_\mu}
\newcommand\vmin{v_\mathsf{min}}

\newcommand\del{\delta}
\newcommand\tstamp{\mathit{T}}
\newcommand\tscol{\mathbb{T}}
\newcommand\dif{\Delta}
\newcommand\uc{\mu C}
\newcommand\holder{\blacklozenge}


We begin with some theoretical foundations then proceed to a practical analysis of delays on the automotive-grade platforms of our setup. 

\subsection{Theoretical background}

Existing definitions from \cite{Moon99} provide sufficient theoretical background on clock offsets, skews and drifts that characterize differences between clock measurements. These were used in the works from \cite{Cho16} for in-vehicle networks, \cite{Kohno05} for computer networks and \cite{Cristea13} for smart-phones over wireless-networks. In all these scenarios, delays are used to identify a particular sender. We stay to the same notions but make small modifications according to our needs. 

Distinct to the case of a general clock-adjustment scenario in computer networks, e.g., \cite{Kohno05} or \cite{Cristea13}, we are missing the time-stamps of each participant and rely only on local clocks. Subsequently, we want to infer on the clock offset based on local timestamps and also from the a-priori knowledge of the precise time intervals at which frames are broadcast. We note that delays are generally fixed in automotive applications and thus we can infer on the intended delay since this is usually a hardcoded constant $10, 50, 100, 500, 1000 \mathit{ms}$, etc.

Figure \ref{fig:clock_skews} shows how the local timestamps are formed and how they account for delays that are expressed as random variables. Whenever principal $\uc_1$ sends a cyclic frame, the frame is sent at delay $\del_{\uc_1}$ which is a random variable that accounts for imperfections in the local clock of $\uc_1$. Subsequently, the frame travels on the bus and propagation delays are accounted which are again represented by a random variable $\del_{\uc_1, \uc_2}$ (the propagation delay includes delays due to arbitration loss or mere propagation of the packet on the bus, etc.). Finally, the time-stamp of the frame is quantized on $\uc_2$ this time accounting for new clock imperfections due to the local clock of $\uc_2$ that are represented in the random variable $\del_{\uc_2}$. In principle, random variable $\del_{\uc_2}$ has a mean that is smaller than the mean of $\del_{\uc_1, \uc_2}$ which can get significantly larger when the busload is high, while the mean of $\del_{\uc_1}$ is much larger than any of the two as it accounts for the delays at which the frame is sent. 

We formally refine the timing metrics that we use in the following definition in attempt to set a theoretical background for our experimental measurements. 


\begin{figure}[t!]
\begin{minipage}{5.8cm}
\centering
\includegraphics[width=5.8 cm]{delay_prop.pdf}
\caption{The travelling time for a frame from $\uc_1$ over the CAN bus to $\uc_2$}
\end{minipage}
\label{fig:ttime}
~
\begin{minipage}{5.8cm}
\centering
\includegraphics[width=5.15 cm]{clock_skews.pdf}
\caption{Offset of the recorded time-stamps in case of ideal clocks}
\end{minipage}
\label{fig:clock_skews}
\end{figure}







\emph{Definition 1.} Let $\dif \tstamp$ be the random variable that accounts for the delay between consecutive occurrences  on the bus of frame identified by its ID sent by principal $\uc_1$ and let $\tscol_{\uc}=\left \{ \dif \tstamp_1, \dif \tstamp_2, ..., \dif \tstamp_n \right \}$ be a recording by principal $\uc_2$ of $n$ consecutive values of variable $\dif \tstamp$, i.e., $\dif \tstamp_i = \tstamp_i-\tstamp_{i-1}, i=1..n, \tstamp_0=0$. We define the following non-random variables that correspond to reference clocks:  
\begin{enumerate}[i.]
\item $\clock^{\refr}_{\real}(t)=t\delta$ where $\delta$ is the intended constant delay between frames, 
\item $\clock^{\refr}_{\mmin} = t \vmin$ where $\vmin$ is the minimum value in $\tscol_{\uc}$,
\item $\clock^{\refr}_{\med} = t \vmed$ where $\vmed$ is the median of the values in $\tscol_{\uc}$,
\item $\clock^{\refr}_{\mean} = t \vmean$ where $\vmean$ is the mean of the values in $\tscol_{\uc}$.
\end{enumerate}

 
Subsequently, we define the cumulative clock offset of principals $\uc_1$ and $\uc_2$ with respect to reference clock $\clock^\refr_{\holder}$ where placeholder $\holder \in \{ \mmin, \mean, \med \}$ as 
$\clock_{\uc_1,\uc_2}(t) - \clock^\refr_{\holder}(t)$ where $\clock_{\uc_1,\uc_2}=\sum_{i=1,t} \dif \tstamp_i$. In the following subsection we analyze the variation of delays with respect to these four reference clocks. While in the protocol description we analyze variations only with respect to $\clock^{\refr}_{\real}$, evaluating the other three clocks should not appear meaningless since without proper evaluation it would have been improper to rule them out as possible indicators.





\subsection{Experimental measurements of delays}

We first perform experiments in order to choose which of the four metrics $\clock^{\refr}_{\real}$, $\clock^{\refr}_{\mmin}$, $\clock^{\refr}_{\med}$, $\clock^{\refr}_{\mean}$ is best suited for our approach. 
We also analyze the case when forced constant delays are added to each packet. For illustration purposes, these delays are fixed to $\pm100$, $\pm250$ and $\pm500$ clock ticks. In case of the TC277 boards (the main actor of our experiments) 1 tick of the  System Timer is the equivalent of 10ns. 
Then we focus on the impact on changing delays by very small variations (in the order of hundreds of clock ticks) on the measurements from the receiver side. Nonetheless we discuss the behavior of lower priority IDs which may lose arbitration and thus add more to the propagation delay. 


Our experimental measurements clearly point toward $\clock^{\refr}_{\real}$ as the best reference value for the clock drift. Indeed, $\clock^{\refr}_{\real}$ is a constant fixed at design time, but it is also easy to determine by empirical evidence on an existing network since manufacturers always choose fixed delays, e.g., 50ms, 100ms.  

We now comment why the other indicators, i.e., $\clock^{\refr}_{\mmin}, \clock^{\refr}_{\med}, \clock^{\refr}_{\mean}$ do not seem to offer a better approximation. The main problem consists in the gap between measurements on a free bus and measurements on a bus that features regular network traffic. We do rely on the minimum, median and mean of the first 100 received packets (by increasing this value the results do improve but not enough to justify the use of these three reference clocks) the subsequent plots are done over the next 1400 frames. When the bus is free of additional traffic the variations between the mean and median values are very small and results computed over a limited number of packets prove to be a bad indicator. The plots appear to be mixed between distinct delays with no obvious separation. This is plotted on the upper side of Figures \ref{fig:skews_mea} and \ref{fig:skews_med}.  When the bus becomes loaded, variations increase by two orders of magnitude and become stable, this is plotted on the lower side of Figures \ref{fig:skews_mea} and \ref{fig:skews_med}. For $\clock^{\refr}_{\mmin}$ apparently there is good separation both in the case of a free bus and a bus that is loaded with regular network traffic, this is depicted in Figure \ref{fig:skews_min}. However, the variations are not correctly aligned with the value of the delay, which suggests that the difference toward the minimum value is again a poor separator. For the same measurements $\clock^{\refr}_{\real}$ proves to be a very good classifier with or without network traffic, measurements are presented in Figure \ref{fig:skews_real}.


In Figures  \ref{fig:skews_mea}, \ref{fig:skews_med}, \ref{fig:skews_min} and \ref{fig:skews_real} we have contrasted between independent measurements on the Infineon board and CANoe since the similarities between the independent measurements prove the correctness of the results. The plots suggest that using the clock drift from a single packet may lead to wrong classifications but the cumulative clock drift computed over a few dozen packets is a very good separator to identify a specific delay. 


\begin{figure}[t!]
\centering
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_mea_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_mea_canoe.png}
\end{minipage}

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_mea_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_mea_canoe.png}
\end{minipage}

\caption{$\clock^{\refr}_{\mean}$ for a frame sent from an Infinenon TC277 as measured on another Infineon board (left) and on CANoe (right) - results over a free bus (up) or with network traffic (down)}
\label{fig:skews_mea}
\end{figure}


\begin{figure}[h!]
\centering
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_med_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_med_canoe.png}
\end{minipage}

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_med_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_med_canoe.png}
\end{minipage}

\caption{$\clock^{\refr}_{\med}$ for a frame sent from an Infinenon TC277 as measured on another Infineon board (left) and on CANoe (right) - results over a free bus (up) or with network traffic (down)}
\label{fig:skews_med}
\end{figure}


\begin{figure}[h!]
\centering
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_min_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_min_canoe.png}
\end{minipage}

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_min_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_min_canoe.png}
\end{minipage}

\caption{$\clock^{\refr}_{\mmin}$ for a frame sent from an Infinenon TC277 as measured on another Infineon board (left) and on CANoe (right) - results over a free bus (up) or with network traffic (down)}
\label{fig:skews_min}
\end{figure}


\begin{figure}[h!]
\centering
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_real_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s1_real_canoe.png}
\end{minipage}

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_real_inf.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{figs/b1_s2_real_canoe.png}
\end{minipage}

\caption{$\clock^{\refr}_{\real}$ for a frame sent from an Infinenon TC277 as measured on another Infineon board (left) and on CANoe (right) - results over a free bus (up) or with network traffic (down)}
\label{fig:skews_real}
\end{figure}

\subsection{Forcing delays on the bus } 

We now discuss the impact on manipulating delays at fine grain clock modifications. This discussion is essential for embedding the authentication values in delays which is the objective of the INCANTA protocol. 

Figure \ref{fig:skews277inf} shows these delays ($\pm100$, $\pm250$ and $\pm500$ clock ticks) when they are measured from another TC277 board without (left)  and with additional traffic (right). In Figure \ref{fig:skews277canoe} we show the same delays when measured from a CANoe/VN device at the same time. Here we choose to present the plot at finer grain by taking only 500 packets, otherwise these plots are consistent with the plots already shown in Figure \ref{fig:skews_real}. The slope of the lines are distinct since the clock of the reference clock from the VN CAN adapter device is distinct. Overlapping the plots in the two cases (with and without traffic) for each reference clock in Figure \ref{fig:skews277over} shows that traffic does not cause significant changes in the clock skew over multiple packets. While small variations can be encountered, the slopes are close for the two cases. 

\begin{figure}[h!]
\centering
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc_297_no_traffic.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc_297_traffic.png}
\end{minipage}

\caption{Delays for a frame sent from an Infinenon TC277 as measured on another Infineon board without (left) and with network traffic (right)}
\label{fig:skews277inf}
\end{figure}



\begin{figure}[h!]
\centering

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc_297_no_traffic_canoe.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc_297_traffic_canoe.png}
\end{minipage}

\caption{Delays for a frame sent from an Infinenon TC277 as measured from CANoe/VN CAN adapter without (left) and with network traffic (right)}
\label{fig:skews277canoe}
\end{figure}



\begin{figure}[h!]
\centering

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc_297_traffic_ovr.png}
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc_297_traffic_canoe_ovr.png}
\end{minipage}

\caption{Delays for a frame sent from an Infinenon TC277 as measured by an Infineon board (left) or from CANoe/VN CAN adapter (right) with and without traffic (overlap)}
\label{fig:skews277over}
\end{figure}



\emph{Low priority IDs}. Switching to low priority IDs leads to significant changes in the delay at which packets arrive. Computed over multiple packets, the clock skew remains the same, but individual packets may come at significant delays.  In Figure \ref{fig:extended} we illustrate delays for one of the TC277 boards in the case with no additional traffic on the bus (i), a bus loaded at 50\% with delays computed on a packet with the highest priority ID (ii) and delays in case of the lowest priority extended ID (iii).  In the later case, it is easy to note that inter-packet delays may have large variations. In part (iv) we overlap these 3 plots and the result confirms that the clock skew is the same for the node. Small variations appear in the case when the delay is set to $0$, $\pm100$ and $\pm250$ between the three cases but the slope of the line that mediates these values is still close, making identification possible. 

\begin{figure}[h!]
\centering

\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc277_clean.png}
\\
(i)
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc277_traffic.png}
\\
(ii)
\end{minipage}


\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc277_extended.png}
\\
(iii)
\end{minipage}
\begin{minipage}{\clpicw cm}
\centering
\includegraphics[width=\lpicw cm]{tc277_all.png}
\\
(iv)
\end{minipage}

\caption{Delays for TC277 on several testbeds: a bus with no traffic (i), with regular traffic and high priority ID (ii) and regular traffic with lowest priority extended ID (iii) and overlap of the three cases (iv) (the slope is similar in all cases)}
\label{fig:extended}
\end{figure}

\emph{Repeated randomized trials.} To get a convincing image on the correctness of the results we proceed to a set of randomized trials that consist in taking small portions of the trace at random positions and compute the variation of clock on the smaller data set. We consider both the case of a free bus and that of a bus loaded with regular network traffic. We performed these tests with 4 Infineon controllers:  TC277, TC297, TC224 and a second TC224. Moreover, these tests are again performed for all the induced delays on packet arrival:  $\pm100$, $\pm250$ and $\pm500$, Figure \ref{fig:skew_all} graphically depicts the results.  For each board the first set of data which is encircled in the figure represent the packet arrival time without any forced delay, the subsequent tests are for plus $100$, $250$ and $500$ ticks and it can be clearly seen that the arrival time increases and is correctly determined by the receiver. Then the delay decreases by $100$, $250$ and $500$ ticks and so does the arrival time measured by the receiver. In the case when regular traffic is present, variations exists due to the obvious fact that the bus may not be free when data is sent and the time-stamp of these packets alone does not offer sufficient information to identify a sender node (or the intended delay).  Fortunately, even with a loaded bus for the majority of packets the delay is correctly estimated as can be seen in  Figure \ref{fig:skew_all}. In the next section we do discuss how to exploit this delay in order to hide authentication information and how additional traffic influences the accuracy of our estimation (some packets do deviate significantly from the expected delay and unavoidably they will contribute to the false positive rate). 


\begin{figure}[h!]
\centering
\centering
\includegraphics[width=12 cm]{figs/skew_all.png}
\caption{Results after 100 tests at randomized locations in the trace for all 4 Infineon controllers:  TC277, TC297, TC224 and a second TC224 and the six added delays $\pm100$, $\pm250$ and $\pm500$ with (right) and without (left) regular network traffic}
\label{fig:skew_all}
\end{figure}


==> experiments.tex <==
\section{Experimental results}


\subsection{Evidencing impersonation using TriCore clock adjustment}

Firstly, we have checked based on the adjustment that we wanted to use which is the most suitable message cyclicity that should be used. Furthermore, we tested how the receiver node counts the time between each two received CAN messages as a multiple of a constant time set at microsecond level. The receiver node will send at the reception of each message the value of the counter so we can compute and estimate the clock skew based on the receiver’s oscillator. 
We have defined the following scenarios, testing without any busload:
\begin{enumerate}
  \item CAN message sent at every 20ms, receiver counter incremented at every 2.5 $\mu$s
  \item CAN message sent at every 100ms, receiver counter incremented at every 2.5 $\mu$s
  \item  CAN message sent at every 100ms, receiver counter incremented at every 1 $\mu$s
  \item CAN message sent at every 1s, receiver counter incremented at every 1 $\mu$s
  \item CAN message sent at every 5s, receiver counter incremented at every 1 $\mu$s
\end{enumerate}

As presented in Figure x3, the third scenario was the one that had fitted best in our approach because we could
compute the clock skew over time in a clear way.

Based on the decision to continue the tests having the CAN message sent every 100ms and the high frequency counter increased every 1us, we have moved forward to the configuration of the timer on the sender node, by adding or substracting multiples of ticks. The strategy was to test the following cases, without busload, and check if the results are satisfactory, so the clock skew could be visibly adjusted if the information from the CAN logs is computed based on the physical time difference shown by the VN1610 in CANoe and the
time difference based on the high frequency counter:
 \renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}
  \item 100ms - 500 ticks
  \item 100ms - 250 ticks
  \item 100ms
  \item 100ms + 250 ticks
  \item 100ms + 500 ticks
\end{itemize}

Only measuring with no busload, the results of the tests were adequate. When we started testing with the replay of a CAN log from a car, creating a bus load, there were two new cases that were added:
 \renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}
  \item 100ms - 100 ticks
  \item 100ms + 100 ticks
\end{itemize}

When we have used the logs with the busload, four units were tested: two TC224s, one TC277 and one TC297. The test duration was, 8-9 minutes for each case and for each unit. The results for all the tests were surprisingly good and based on them we have the evidenced that the impersonation of an authentic unit is possible by adjusting the cyclicity of the message using the high precision timer from the TriCore. Externally, this would be visible as a different clock skew every time so that, by using this method, one unit with the configuration we have used can be the clone or the replacement of an existing unit from a real vehicle.

\begin{figure}[t!]
\centering
\includegraphics[width=8 cm]{CAN_Log3_measurements.png}
\caption{CAN message sent at every 100ms, receiver counter incremented at every 1 $\mu$s}
\label{fig:clock_skews}
\end{figure}

\subsection{Authentication protocol based on clock skew}

In our understanding, the authentication methods proposed or used in real-time situations
presented in [2], [3], [4], [5] or [6] are resource and time consuming:
\renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}
  \item  Using shared cryptographic keys and applying MACs on the message data bytes
  \item  Message digest applied on a random seed and verification of message parts by two or more ECUs for ensuring mutual authentication
  \item  Firewalls added between critical units and the bus
\end{itemize}

Additionally to the implementation presented in subchapter 3.2, we have considered a new approach and have implemented the following steps:
\renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}
  \item  Increase an internal 32 bit counter on the sender side after every sent message and update the least significant 4 bytes of the data bytes with the counter value
  \item  Compute an internal adjustment of the timer based on the MD5 hash function applied to this counter and use the last 17 bits of the result to adjust the message ciclicity (most significant bit is the $ Sign_{bit} $ and the remaining 16 bits represents the adjustment value, in ticks called $ Ticks_{TimerAdjustment}) $
  \item  Reconfigure the timer to generate an interrupt based on the following equations

\begin{equation}
New_{TimerAdjustment} = Ticks_{100ms} \pm Ticks_{TimerAdjustment}
\end{equation}

where the sign of 

\begin{equation}
Ticks_{TimerAdjustment}
\end{equation}

depends on the following condition

$$
sign=
\begin{cases}
+, & \text { if } Sign_{bit} \ is \ 1\\
-, & \text { if } Sign_{bit} \ is \ 0\\
\end{cases}
$$

\end{itemize}

The test results for this approach have shown that this type of time covert channel authentication is possible, with an error evaluated to x1\% in a number of y cases. The possibility for an adversary to tamper the authentication is estimated at x2\%, which can still be considered as a potential problem. Further, we considered that we can try to use more than 16 bits from the MD5 result as a timer adjustment value. We have tested with 18 bits and 20 bits and the results were satisfactory and the chance that an adversary can fraud the authentication was below 1\%.

In addition to the mentioned, we have used SHA256 instead of MD5 but increased the message cyclicity from 100ms to 1s and also increased the timer adjustment size to 22 bits, 24 bits and 26 bits. In this case, the results were great but the necesarry time for the authentication to be done was considered problematic.

\subsection{Security improvements for the authentication protocol}


In order to reduce the cases of authentication problems due to high bus load, we have considered an improvement for the method described in subchapter 3.3. The update is ongoing as work and tests and consists of the following steps :
\renewcommand{\labelitemi}{$\bullet$}
\begin{itemize}
  \item  Increase an internal 32 bit counter on the sender side after every sent message and
update the least significant 4 bytes of the data bytes with the counter value
  \item  Reconfigure the timer to generate an interrupt based on the following equations

\begin{equation}
New_{TimerAdjustment} = Ticks_{20{\mu}s}
\end{equation}
   Check $ CAN_{TXRQ} $, and if
   \renewcommand{\labelitemi}{$\square$}
   \begin{itemize}
	\item  flag is set to 1, increase an internal repetition counter and repeat the step before
	\item flag is set to 0 compute an internal adjustment of the timer based on the SHA256 hash function applied to this counter and use the last 17 bits of the result to adjust the message ciclicity (most significant bit is the sign bit and the remaining 16 bits represents the adjustment value, in ticks)
	\renewcommand{\labelitemi}{$\asterisk$}
   	\begin{itemize}
		\item 
		
		\begin{equation}
		\mathit{If} \ \mathit{Ticks}_{20{\mu}s} \times Repetition_{Counter} > Defined_{Threshold}, then
		\end{equation}
		
		\begin{equation}
		New_{TimerAdjustment} = Ticks_{20{\mu}s}  \times Repetition_{Counter} + 2^{Sign_{bit}}  \times  Ticks_{TimerAdjustment}
		\end{equation}
		and send a new message with the authentication tag.After the message is sent, set
		\begin{multline}
		New_{TimerAdjustment} = Ticks_{100ms} - Ticks_{20{\mu}s}  \times Repetition_{Counter} \\ 
		 - 2^{Sign_{bit}}   \times  Ticks_{TimerAdjustment}  \pm Ticks_{TimerAdjustment}
		\end{multline}
		where the sign of 
		\begin{equation}
		Ticks_{TimerAdjustment}
		\end{equation}
		depends on the following condition
		$$
		sign=
		\begin{cases}
		+, & \text { if } Sign_{bit} \ is \ 1\\
		-, & \text { if } Sign_{bit} \ is \ 0\\
		\end{cases}
		$$
		\item
		\begin{equation}
		Else, \ New_{TimerAdjustment} = Ticks_{100ms} \pm Ticks_{TimerAdjustment}
		\end{equation}
		where the sign of 
		\begin{equation}
		Ticks_{TimerAdjustment}
		\end{equation}
		depends on the following condition
		$$
		sign=
		\begin{cases}
		+, & \text { if } Sign_{bit} \ is \ 1\\
		-, & \text { if } Sign_{bit} \ is \ 0\\
		\end{cases}
		$$
	\end{itemize}
    \end{itemize}
\end{itemize}
